Unsupervised Speech Decomposition via Triple Information Bottleneck

Speech information can be roughly decomposed into four components: language content, timbre, pitch, and rhythm. Obtaining disentangled representations of these components is useful in many speech analysis and generation applications. Recently, state-of-the-art voice conversion systems have led to speech representations that can disentangle speaker-dependent and independent information. However, these systems can only disentangle timbre, while information about pitch, rhythm and content is still mixed together. Further disentangling the remaining speech components is an under-determined problem in the absence of explicit annotations for each component, which are difficult and expensive to obtain. In this paper, we propose SpeechSplit, which can blindly decompose speech into its four components by introducing three carefully designed information bottlenecks. SpeechSplit is among the first algorithms that can separately perform style transfer on timbre, pitch and rhythm without text labels. Our code is publicly available at https://github.com/auspicious3000/SpeechSplit.

==> sections/intro_old.tex <==
% As the most unique means of communication among humans, speech conveys rich information. The primary goal of speech is to express language content, which, in most cases, can be transcribed to text. However, speech contains a lot of other information beyond its text transcriptions. First, the timbre of speech, or commonly known as the voice characteristics, conveys the speaker identity information. Second, the prosody of speech, which involves both pitch variations and rhythm, conveys the emotion of the speaker. In summary, as shown in figure **, speech information can be roughly decomposed into three aspects: \emph{language content}, \emph{timbre} and \emph{prosody} (which includes \emph{pitch} and \emph{rhythm}). Moreover, except for the language content, which can arguably be considered as \emph{speaker-independent}, the other aspects are generally considered as \emph{speaker-dependent} -- each speaker has his/her own voice characteristics, intonation, and preferred pace of talking.

% For decades, speech researchers have been studying the problem of voice conversion, whose goal is to convert a given source speech by replacing its speaker-dependent information with that of a target speaker. In recent years, deep style transfer algorithms have been applied to voice conversion without parallel training data, where each speaker is regarded as a \emph{domain}, and the speaker-dependent information is regarded as the \emph{domain style}. Although the specific algorithms vary, many style transfer methods share one common principle, which is to obtain a domain-invariant feature, which disentangles all the speaker-dependent information. The domain-invariant feature is then fed into a domain-specific decoder to generate speech that matches the speech distribution in that domain. In this paper, we will refer to these methods as \emph{voice style transfer} methods.

% Despite their initial success, existing voice style transfer algorithms have been suffering from one mysterious failure. Since these algorithms are designed to disentangle all speaker-dependent information, they should supposedly be able to convert both timbre and prosody. However, while timbre can be very well disentangled and converted, few existing voice style transfer algorithms are able to convert prosody, particularly the rhythm aspect. In most cases, the source speech and the converted speech are perfectly aligned in time, even if the source speaker is a slow speaker and the target speaker is a fast speaker.

As the most unique means of communication among humans, speech conveys rich information. As shown in figure **, speech information can be roughly decomposed into three aspects: \emph{language content}, which can also be transcribed to text, \emph{timbre}, which reveals speaker identity, and \emph{prosody}, including \emph{pitch} and \emph{rhythm}, which conveys the emotion of the speaker. In particular, rhythm characterizes the pace at which each word is utterred, and is the only aspect that is closely related to time. Among these aspects, language content can arguably be considered as \emph{speaker-independent}, while the other aspects are generally considered as \emph{speaker-dependent} -- each speaker has his/her own voice characteristics, intonation, and pace of talking.

For decades, speech researchers have been studying the problem of voice conversion, whose goal is to convert a given source speech by replacing its speaker-dependent information with that of a target speaker. In recent years, deep style transfer algorithms have been applied to voice conversion without parallel training data. Although the specific algorithms vary, many style transfer methods share one common principle, which is to obtain a domain-invariant feature, which disentangles all the speaker-dependent information. %The domain-invariant feature is then fed into a domain-specific decoder to generate speech that matches the speech distribution in that domain. In this paper, we will refer to these methods as \emph{voice style transfer} methods.

Despite their success, the existing voice style transfer algorithms have one limitation. 
% Since both timbre and prosody are speaker-dependent, these algorithms should desirably convert both timbre and prosody. However, 
While timbre can be very well disentangled and converted, few existing algorithms are able to convert prosody, particularly the rhythm aspect. In most cases, the source speech and the converted speech are perfectly aligned in time, even if the source speaker is a slow speaker and the target speaker is a fast speaker.

Inspired by an information-theoretic perspective on style transfer and disentanglement proposed in **, one can identify a plausible cause of the failure in prosody conversion. According to this perspective, the key to an ideal disentanglement of an aspect is the availability of a label that preserves all the information of this aspect. In voice conversion, we have access to the speaker identity, which is almost a one-to-one mapping to timbre, and therefore timbre disentanglement is successful. On the other hand, speaker identity is only very loosely connected to prosody, and therefore existing style transfer approaches cannot disentangle prosody. 

As an imprecise analogy, consider solving the unknowns of an equation \e{c+t+p=16}, where \e{c} stands for content, \e{t} stands for timbre and \e{p} stands for prosody. With access to the information of \e{t}, \emph{e.g.} \e{t=5}, a style transfer algorithm can `subtract' the information from both sides of the equation, leading to a representation that is invariant to \e{t}, but still lumps \e{c} and \e{p} together, \emph{i.e.} \e{c+p=11}. Therefore, in order to further disentangle prosody from the language content, one would need an information-preserving label for either prosody \e{p} or the language content \e{c}. 

However, obtaining the labels for the two aspects have their respective difficulties. As for the prosody labels, notice that prosody consists of pitch and rhythm. While the pitch label can be easily obtained by pitch tracking algorithms **, it is unclear what constitutes the rhythm label, not to mention how to obtain the label. As will be shown in this paper, we have experimented with different hand-crafted rhythm labels, but none of them contains adequate information to disentangle rhythm. On the other hand, the language content label is well-defined as the text transcriptions. In fact, there have been many algorithms ** that force prosody disentanglement with the supervision of text transcriptions. However, these algorithms are language specific, and obtaining large number of of text transcriptions is expensive, especially for low-resourced languages. Therefore, we will focus on unsupervised methods that do not rely on text transcriptions.

As a result, we have run into the crux of disentangling time. Without resorting to extra supervision, disentangling the rhythm aspect is under-determined, just like solving two unknowns with only one equation. The only knowledge we have about rhythm is that it is correlated with time, while other aspects is not. Hence, here comes our research question: is it possible to blindly decompose these remaining aspects in speech in an unsupervised manner based on our limited knowledge of the rhythm aspect?

In this paper, we propose \algnamens, a versatile voice conversion algorithm that can decompose speech into the language content, timbre, pitch and rhythm. Thus, \algname is among the first voice conversion algorithms that can separately convert different aspects to different styles. In other words, it can flexibly convert timbre to one speaker style, and prosody to another style. \algname does not rely on any text transcription. Instead, it introduces an encoder-decoder structure with three channels with different information bottleneck designs. It turns out that the difference in the information bottleneck is able to force different channels to pass different information -- one passes the language content and the other passes rhythm, and thereby achieves the blind disentanglement between these two aspects. \algname also reveals some intriguing behaviors of deep neural networks in the presence of information bottleneck.

% \algname also reveals some intriguing behaviors of deep neural networks in the presence of information bottleneck, which strengthens and supplements the claims in **. In **, it is observed that when there is one information bottleneck and some essential information supplied \emph{after} the bottleneck, then the neural network will squeeze out such information before passing the information bottleneck, because such information will be supplied anyway after the bottleneck. In this paper, we will show that when multiple information bottlenecks are present, each information bottleneck will squeeze out the information that would be easier to pass in the other bottlenecks. These findings provide valuable insights on how neural networks process information.
